On the Higgs spectra of the 3-3-1 model with the sextet of scalars engendering the type II seesaw mechanism

In the 3-3-1 model with right-handed neutrinos, three triplets of scalars engender the correct sequence of symmetry breaking, $SU(3)_C \times SU(3)_L \times U(1)_X \rightarrow SU(3)_C \times SU(2)_L \times U(1)_Y \rightarrow SU(3)_C \times U(1)_{EM}$, generating mass for all fermions, except neutrinos. Tiny neutrino masses may be achieved by adding one sextet of scalars to the original scalar content. As consequence, it emerges a very complex scalar sector, involving terms that violate lepton number explicitly, too. The main obstacle to the development of the phenomenology of such scenario is the knowledge of its spectrum of scalars since, now, there are 15 massive scalar particles on it. The proposal of this work is to do an exhaustive analysis of such scalar sector with lepton number being explicitly violated at low, electroweak and high energy scales by means of trilinear terms in the potential. The first case can be addressed analytically and, as a nice result, we have observed that the scalar content of such case is split into two categories: One belonging to the 331 energy scale and the other belonging to the EWSB energy scale, with the last recovering the well known THDM+triplet. For the other cases, the scalar sector can be addressed only numerically. Hence, we proposed a very general approach for the numerical study of the potential, avoiding simplifications that can make us reach conclusions without foundation. We show that, in the case of lepton number being explicitly violated at electroweak scale, it is possible to recover the same physics of the THDM+triplet, as the previous case. Among all the possibilities, we call the attention to one special case which generates the 3HDM+triplet scenario. For the last case, when lepton number is violated at high energy scale, the sextet become very massive and decouples from the original scalar content of the 3-3-1 model.

==> rascunho.tex <==

\subsection{$M_1,M_2\gg f\sim v$}

The last case is related with the almost total decoupling of the sextet scalar particles. Here, such energy scale for $M_1$ and $M_2$ simulates a simple THDM. The THDM is simulated by the singly-charged scalar $h_1^\pm$, the pseudoscalar $A_1$ and  two CP-even scalars $h_1$ (the Higgs) and $h_5$. 
The most interesting result for $M_1,\;M_2\gg f \sim v$ is that, even for a regime in which the explicitly leptonic symmetry breaking scale $M_1,\;M_2$ is high, the scalar predominantly $R_\Delta$ decouples from the other particles and it is heavy as the CP-even predominantly $R_\sigma$. Then, all the sextet particles totally decouples from the other particles of the model.


\begin{figure}[ht] 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering\includegraphics[width=0.75\linewidth]{figuras/mr11_ew3.pdf} 
    \label{fig3b:a} 
    \vspace{4ex}
  \end{subfigure}%% 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
\includegraphics[width=0.75\linewidth]{figuras/mr12_ew3.pdf} 
    %\caption{Rupture} 
    \label{fig3b:b} 
    \vspace{4ex}
  \end{subfigure} 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering    \includegraphics[width=0.75\linewidth]{figuras/mr13_ew.pdf}
    %\caption{DFT, Initial condition} 
    \label{fig3b:c} 
  \end{subfigure}%%
\caption{CP even $M_1,M_2\gg f\sim v$ . The blue dots represents all possible positive definite masses of the scalars at tree-level and the red dots represents the positive definite masses of the scalars with the Higgs-like particle mass ($m_{h_1}$) lying between $100$ GeV and $200$ GeV(See the text).}
  \label{fig3b} 
\end{figure}



However, for the CP-odd sector, there is a total decoupling of the $A_2$ pseudoscalar, since its mass depends directly on the explicitly symmetry breaking scales $M_1,\;M_2$. Hence, for the CP-odd sector, the only phenomenological viable particle is the $A_1$, predominantly a composition between $I_\rho$ and $I_\eta$.

\begin{figure}[ht] 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering    \includegraphics[width=0.75\linewidth]{figuras/ma11_ew3.pdf}    %\caption{Initial condition}    
    \label{fig6b:a} 
    \vspace{4ex}
  \end{subfigure}%% 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
\includegraphics[width=0.75\linewidth]{figuras/ma12_ew3.pdf}   %\caption{Rupture} 
    \label{fig6b:b} 
    \vspace{4ex}
  \end{subfigure} 
 \caption{CP odd $M_1,M_2\gg f\sim v$. The blue dots represents all possible positive definite masses of the scalars at tree-level and the red dots represents the positive definite masses of the scalars with the Higgs-like particle mass ($m_{h_1}$) lying between $100$ GeV and $200$ GeV(See the text). }
  \label{fig6b} 
\end{figure}








\begin{figure}[ht] 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering    \includegraphics[width=0.75\linewidth]{figuras/mc11_ew3.pdf}    %\caption{Initial condition}    
\caption{331 singly-charged scalars} 
    \label{fig9b:a} 
    \vspace{4ex}
  \end{subfigure}%% 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
\includegraphics[width=0.75\linewidth]{figuras/mc21_ew3.pdf}   %\caption{Rupture} 
\caption{EW singly-charged scalars} 
    \label{fig9b:b} 
    \vspace{4ex}
  \end{subfigure} 
 \caption{Singly charged scalars $M_1,M_2\gg f\sim v$. The blue dots represents all possible positive definite masses of the scalars at tree-level and the red dots represents the positive definite masses of the scalars with the Higgs-like particle mass ($m_{h_1}$) lying between $100$ GeV and $200$ GeV(See the text).}
  \label{fig9b} 
\end{figure}

The same happens for the singly-charged sector. The charged scalar predominantly $\Delta^\pm$ decouples totally from the $h_1^\pm$ scalar and becomes very heavy due the scale of $M_1$ and $M_2$. The same happens for the doubly-charged scalar. 


\begin{figure}[ht] 
    \centering    \includegraphics[width=0.4\linewidth]{figuras/md11_ew3.pdf}    \caption{$M_1,M_2\gg f\sim v$  Doubly charged scalar. The blue dots represents all possible positive definite masses of the scalars at tree-level and the red dots represents the positive definite masses of the scalars with the Higgs-like particle mass ($m_{h_1}$) lying between $100$ GeV and $200$ GeV(See the text).}    
    \vspace{4ex}
  \label{fig12b} 
\end{figure}




\begin{figure}[ht] 
    \centering    \includegraphics[width=0.4\linewidth]{figuras/mr21_ew3.pdf}    \caption{$M_1,M_2\gg f\sim v$  Complex neutral scalar. The blue dots represents all possible positive definite masses of the scalars at tree-level and the red dots represents the positive definite masses of the scalars with the Higgs-like particle mass ($m_{h_1}$) lying between $100$ GeV and $200$ GeV(See the text).}    
    \vspace{4ex}
  \label{fig15b} 
\end{figure}
%%%%%%

\clearpage


